Response-G1: Explicit Scene Graph Modeling for Proactive Streaming Video Understanding

Proactive streaming video understanding requires Video-LLMs to decide when to respond as a video unfolds, a task where existing methods often fall short due to their implicit, query-agnostic modeling of visual evidence. We introduce Response-G1, a novel framework that establishes explicit, structured alignment between the accumulated video evidence and the query's expected response conditions via scene graphs. The framework operates in three fine-tuning-free stages: (1) online query-guided scene graph generation from streaming clips; (2) memory-based retrieval of the most semantically relevant historical scene graphs; and (3) retrieval-augmented trigger prompting for per-frame "silence/response" decisions. By grounding both evidence and conditions in a shared graph representation, Response-G1 achieves more interpretable and accurate response timing decisions. Experimental results on established benchmarks demonstrate the superiority of our method in both proactive and reactive tasks, validating the advantage of explicit scene graph modeling and retrieval in streaming video understanding.

==> sec/table.tex <==
\begin{table*}[t]
\centering
% \Huge
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Params}}} & \multicolumn{11}{c|}{\textbf{Real-Time   Visual Understanding}}                                                                                                                 & \multicolumn{5}{c|}{\textbf{Omni-Source   Understanding}}                                  & \multicolumn{5}{c|}{\textbf{Contextual   Understanding}}                                     & \multirow{2}{*}{\textbf{Overall}} \\ \cline{3-23}
                                & \multicolumn{1}{c|}{}                                 & \textbf{OP} & \textbf{CR} & \textbf{CS} & \textbf{ATP} & \textbf{EU} & \textbf{TR} & \textbf{PR} & \textbf{SU} & \textbf{ACP} & \textbf{CT} & \multicolumn{1}{c|}{\textbf{All}} & \textbf{ER} & \textbf{SCU} & \textbf{SD} & \textbf{MA} & \multicolumn{1}{c|}{\textbf{All}} & \textbf{ACU} & \textbf{MCU} & \textbf{SQA} & \textbf{PO} & \multicolumn{1}{c|}{\textbf{All}} &                                   \\ \hline
\multicolumn{24}{c}{\textbf{Human}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
Human                           & \multicolumn{1}{c|}{-}                                & 89.5        & 92.0        & 93.6        & 91.5         & 95.7        & 92.5        & 88.0        & 88.8        & 89.7         & 91.3        & \multicolumn{1}{c|}{91.5}         & 88.0        & 88.2         & 93.6        & 90.3        & \multicolumn{1}{c|}{90.3}         & 88.8         & 90.4         & 95.0         & 100       & \multicolumn{1}{c|}{93.6}         & 91.7                              \\ \hline
\multicolumn{24}{c}{\textbf{Proprietary MLLMs}}                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
Claude 3.5 Sonnet~\cite{anthropic2024claude}               & \multicolumn{1}{c|}{-}                                & 80.5        & 77.3        & 82.0        & 81.7         & 72.3        & 75.4        & 61.1        & 61.8        & 69.3         & 43.1        & \multicolumn{1}{c|}{72.4}         & 31.6        & 34.0         & 32.8        & 48.8        & \multicolumn{1}{c|}{36.8}         & 38.4         & 34.8         & 34.4         & 64.7        & \multicolumn{1}{c|}{37.7}         & 57.7                              \\
GPT-4o~\cite{hurst2024gpt}                          & \multicolumn{1}{c|}{-}                                & 77.1        & 80.5        & 83.9        & 76.5         & 70.2        & 83.8        & 66.7        & 62.2        & 69.1         & 49.2        & \multicolumn{1}{c|}{73.3}         & 41.2        & 37.2         & 43.6        & 56.0        & \multicolumn{1}{c|}{44.5}         & 41.2         & 38.4         & 32.8         & 56.9        & \multicolumn{1}{c|}{38.7}         & 60.2                              \\
Gemini 1.5 pro~\cite{team2024gemini}                  & \multicolumn{1}{c|}{-}                                & 79.0        & 80.5        & 83.5        & 79.7         & 80.0        & 84.7        & 77.8        & 64.2        & 72.0         & 48.7        & \multicolumn{1}{c|}{75.7}         & 46.8        & 39.6         & 74.9        & 80.0        & \multicolumn{1}{c|}{60.2}         & 51.4         & 40.7         & 54.8         & 45.1        & \multicolumn{1}{c|}{48.7}         & 67.1                              \\ \hline
\multicolumn{24}{c}{\textbf{Open-Source   Video-LLMs}}                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
Video-LLaMa2~\cite{cheng2024videollama}                    & \multicolumn{1}{c|}{7B}                               & 55.9        & 55.5        & 57.4        & 58.2         & 52.8        & 43.6        & 39.8        & 42.7        & 45.6         & 35.2        & \multicolumn{1}{c|}{49.5}         & 30.4        & 32.4         & 30.4        & 36.0        & \multicolumn{1}{c|}{32.4}         & 24.8         & 26.8         & 18.7         & 0.0         & \multicolumn{1}{c|}{21.9}         & 40.4                              \\
VILA-1.5~\cite{lin2024vila}                        & \multicolumn{1}{c|}{8B}                               & 53.7        & 48.2        & 71.0        & 56.9         & 43.4        & 53.9        & 54.6        & 48.8        & 50.1         & 17.6        & \multicolumn{1}{c|}{52.3}         & 41.6        & 26.4         & 28.4        & 36.0        & \multicolumn{1}{c|}{33.1}         & 26.8         & 34.0         & 23.2         & 17.7        & \multicolumn{1}{c|}{27.4}         & 43.2                              \\
Video-CCAM~\cite{fei2024video}                      & \multicolumn{1}{c|}{14B}                              & 56.4        & 57.8        & 65.3        & 62.8         & 64.6        & 51.4        & 42.6        & 48.0        & 49.6         & 31.6        & \multicolumn{1}{c|}{54.0}         & 33.6        & 22.0         & 28.4        & 34.8        & \multicolumn{1}{c|}{29.7}         & 27.6         & 24.4         & 16.7         & 22.7        & \multicolumn{1}{c|}{22.9}         & 42.5                              \\
LongVA~\cite{zhang2024long}                          & \multicolumn{1}{c|}{7B}                               & 70.0        & 63.3        & 61.2        & 70.9         & 62.7        & 59.5        & 61.1        & 53.7        & 54.7         & 34.7        & \multicolumn{1}{c|}{60.0}         & 39.6        & 32.4         & 28.0        & 41.6        & \multicolumn{1}{c|}{35.4}         & 32.8         & 29.6         & 30.3         & 15.9        & \multicolumn{1}{c|}{30.0}         & 48.7                              \\
InternVL-V2~\cite{chen2024far}                     & \multicolumn{1}{c|}{8B}                               & 68.1        & 60.9        & 96.4        & 77.1         & 67.7        & 62.9        & 59.3        & 53.3        & 55.0         & 56.5        & \multicolumn{1}{c|}{63.7}         & 37.6        & 26.4         & 37.2        & 42.0        & \multicolumn{1}{c|}{35.8}         & 32.0         & 31.2         & 32.3         & 40.9        & \multicolumn{1}{c|}{.32.42}       & 51.4                              \\
Kangaroo~\cite{liu2024kangaroo}                        & \multicolumn{1}{c|}{7B}                               & 71.1        & 84.4        & 70.7        & 73.2         & 67.1        & 61.7        & 56.5        & 55.7        & 62.0         & 38.9        & \multicolumn{1}{c|}{64.6}         & 37.6        & 31.2         & 28.8        & 39.2        & \multicolumn{1}{c|}{34.2}         & 32.8         & 26.4         & 33.8         & 16.0        & \multicolumn{1}{c|}{30.1}         & 51.1                              \\
LLaVA-NeXT-Video~\cite{liu2024llavanext}                & \multicolumn{1}{c|}{32B}                              & 78.2        & 70.3        & 73.8        & 76.8         & 63.4        & 69.8        & 57.4        & 56.1        & 64.3         & 38.9        & \multicolumn{1}{c|}{67.0}         & 37.7        & 24.8         & 34.4        & 42.8        & \multicolumn{1}{c|}{34.9}         & 29.2         & 30.4         & 35.4         & 18.2        & \multicolumn{1}{c|}{30.8}         & 52.8                              \\
MiniCPM-V-2.6~\cite{hu2024minicpm}                   & \multicolumn{1}{c|}{8B}                               & 71.9        & 71.1        & 77.9        & 75.8         & 64.6        & 65.7        & 70.4        & 56.1        & 62.3         & 53.4        & \multicolumn{1}{c|}{67.4}         & 40.8        & 24.0         & 34.0        & 41.2        & \multicolumn{1}{c|}{35.0}         & 34.0         & 31.6         & 41.9         & 22.2        & \multicolumn{1}{c|}{35.0}         & 53.9                              \\
LLaVA-OneVision~\cite{li2024llava}                 & \multicolumn{1}{c|}{7B}                               & 80.4        & 74.2        & 76.0        & 80.7         & 72.7        & 71.7        & 67.6        & 65.5        & 65.7         & 45.1        & \multicolumn{1}{c|}{71.1}         & 40.8        & 37.2         & 33.6        & 44.8        & \multicolumn{1}{c|}{38.4}         & 35.6         & 36.0         & 27.3         & 29.6        & \multicolumn{1}{c|}{32.7}         & 56.4                              \\
Qwen2-VL~\cite{bai2025qwen2}                      & \multicolumn{1}{c|}{7B}                               & 75.2        & 82.8        & 73.2        & 77.5         & 68.3        & 71.0        & 72.2        & 61.2        & 61.5         & 46.1        & \multicolumn{1}{c|}{69.0}         & 41.2        & 22.0         & 32.8        & 46.6        & \multicolumn{1}{c|}{34.9}         & 31.2         & 26.0         & 39.6         & 22.7        & \multicolumn{1}{c|}{31.7}         & 54.1                              \\ \hline
\multicolumn{24}{c}{\textbf{Open-Source   Streaming Video-LLMs}}                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
Flash-VStream~\cite{zhang2025flash}                   & \multicolumn{1}{c|}{7B}                               & 25.9        & 43.6        & 24.9        & 23.9         & 27.3        & 13.1        & 18.5        & 25.2        & 23.9         & 48.7        & \multicolumn{1}{c|}{23.2}         & 25.9        & 24.9         & 25.6        & 28.4        & \multicolumn{1}{c|}{26.0}         & 24.8         & 25.2         & 26.8         & 2.0         & \multicolumn{1}{c|}{24.1}         & 24.0                              \\
VideoLLM-online~\cite{chen2024videollm}                 & \multicolumn{1}{c|}{8B}                               & 39.1        & 40.1        & 34.5        & 31.1         & 46.0        & 32.4        & 31.5        & 34.2        & 42.5         & 27.9        & \multicolumn{1}{c|}{36.0}         & 31.2        & 26.5         & 24.1        & 32.0        & \multicolumn{1}{c|}{28.5}         & 24.2         & 29.2         & 30.8         & 3.9         & \multicolumn{1}{c|}{26.6}         & 32.5                              \\
Dispider~\cite{qian2025dispider}                        & \multicolumn{1}{c|}{7B}                               & 74.9        & 75.5        & 74.1        & 73.1         & 74.4        & 89.9        & 76.2        & 62.9        & 62.2         & 45.8        & \multicolumn{1}{c|}{67.6}         & 35.5        & 25.3         & 38.6        & 43.6        & \multicolumn{1}{c|}{35.7}         & 39.6         & 27.7         & 34.8         & 25.3        & \multicolumn{1}{c|}{33.6}         & 53.1                              \\
TimeChat-Online~\cite{yao2025timechat}                 & \multicolumn{1}{c|}{7B}                               & 80.2        & 82.0        & 79.5        & 83.3         & 76.1        & 78.5        & 78.7        & 64.6        & 69.6         & 58.0        & \multicolumn{1}{c|}{75.4}         & 38.4        & 26.8         & 35.6        & 50.4        & \multicolumn{1}{c|}{37.8}         & 39.2         & 31.6         & 41.6         & 28.8        & \multicolumn{1}{c|}{35.3}         & 58.1                              \\
StreamAgent~\cite{yang2025streamagent}                     & \multicolumn{1}{c|}{7B}                               & 79.6        & 78.3        & 79.3        & 75.9         & 74.7        & 76.9        & 82.9        & 66.3        & 73.7         & 55.4        & \multicolumn{1}{c|}{74.3}         & 35.9        & 26.3         & 38.9        & 44.0        & \multicolumn{1}{c|}{36.3}         & 39.7         & 30.3         & 39.6         & 28.9        & \multicolumn{1}{c|}{34.6}         & 57.0                              \\ \hline
Response-G1                     & \multicolumn{1}{c|}{8B}                               & 83.3        & 80.2        & 79.6        & 80.6         & 74.5        & 81.6        & 79.2        & 63.2        & 70.9         & 58.3        & \multicolumn{1}{c|}{75.1}         & 36.5        & 29.2         & 39.3        & 43.4        & \multicolumn{1}{c|}{37.1}         & 39.8         & 32.6         & 39.3         & 44.7        & \multicolumn{1}{c|}{39.1}         & 58.7                              \\ \hline
\end{tabular}
}
\caption{Performance comparison on StreamingBench.
Following the official benchmark settings, the PO (Proactive Output) subtask implemented using \textit{proactive} interaction mode, requiring the model to determine when to respond in the video stream.
All other subtasks follow the \textit{reactive} interaction mode, where the response timing is provided.}
\label{table:streamingbench}
\end{table*}







\begin{table*}[t]
\centering
% \Huge
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccccccccccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Params}}} & \multicolumn{7}{c|}{\textbf{Real-Time Visual Perception}}                                                                   & \multicolumn{4}{c|}{\textbf{Backward Tracing}}                                 & \multicolumn{4}{c|}{\textbf{Forward Active Responding}}                        & \multirow{2}{*}{\textbf{Overall}} \\ \cline{3-17}
                                & \multicolumn{1}{c|}{}                                 & \textbf{OCR} & \textbf{ACR} & \textbf{ATR} & \textbf{STU} & \textbf{FPD} & \textbf{OJR} & \multicolumn{1}{c|}{\textbf{Avg.}} & \textbf{EPM} & \textbf{ASI} & \textbf{HLD} & \multicolumn{1}{c|}{\textbf{Avg.}} & \textbf{REC} & \textbf{SSR} & \textbf{CRR} & \multicolumn{1}{c|}{\textbf{Avg.}} &                                   \\ \hline
\multicolumn{18}{c}{\textbf{Human}}                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
Human                           & \multicolumn{1}{c|}{-}                                & 94           & 92.6         & 94.8         & 92.7         & 91.1         & 94           & \multicolumn{1}{c|}{93.2}         & 92.6         & 93           & 91.4         & \multicolumn{1}{c|}{92.3}         & 95.5         & 89.7         & 93.6         & \multicolumn{1}{c|}{92.9}         & 92.8                              \\ \hline
\multicolumn{18}{c}{\textbf{Proprietary MLLMs}}                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
GPT-4o~\cite{hurst2024gpt}                          & \multicolumn{1}{c|}{-}                                & 69.1         & 65.1         & 65.5         & 50           & 68.3         & 63.7         & \multicolumn{1}{c|}{63.6}         & 49.8         & 71           & 55.4         & \multicolumn{1}{c|}{58.7}         & 27.6         & 73.2         & 59.4         & \multicolumn{1}{c|}{53.4}         & 58.6                              \\
Gemini 1.5 Pro~\cite{team2024gemini}                  & \multicolumn{1}{c|}{-}                                & 87.3         & 67           & 80.2         & 54.5         & 68.3         & 67.4         & \multicolumn{1}{c|}{70.8}         & 68.6         & 75.7         & 52.7         & \multicolumn{1}{c|}{62.3}         & 35.5         & 74.2         & 61.7         & \multicolumn{1}{c|}{57.2}         & 65.3                              \\ \hline
\multicolumn{18}{c}{\textbf{Open-Source   Video-LLMs}}                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
LongVU~\cite{shen2024longvu}                          & \multicolumn{1}{c|}{7B}                               & 55.7         & 49.5         & 59.5         & 48.3         & 68.3         & 63           & \multicolumn{1}{c|}{57.4}         & 43.1         & 66.2         & 9.1          & \multicolumn{1}{c|}{39.5}         & 16.6         & 69           & 60           & \multicolumn{1}{c|}{48.5}         & 48.5                              \\
InternVL-V2~\cite{chen2024far}                     & \multicolumn{1}{c|}{8B}                               & 68.5         & 58.7         & 69           & 44.9         & 67.33        & 56           & \multicolumn{1}{c|}{60.7}         & 43.1         & 61.5         & 27.4         & \multicolumn{1}{c|}{44}           & 25.8         & 57.6         & 52.9         & \multicolumn{1}{c|}{45.4}         & 50.1                              \\
Qwen2-VL~\cite{wang2024qwen2}                        & \multicolumn{1}{c|}{7B}                               & 69.1         & 53.2         & 63.8         & 50.6         & 66.3         & 60.9         & \multicolumn{1}{c|}{60.7}         & 44.4         & 66.9         & 34.4         & \multicolumn{1}{c|}{48.6}         & 30.1         & 65.7         & 50.8         & \multicolumn{1}{c|}{48.9}         & 52.7                              \\
LLaVA-OneVision~\cite{li2024llava}                 & \multicolumn{1}{c|}{7B}                               & 67.1         & 58.7         & 69.8         & 49.4         & 71.3         & 60.3         & \multicolumn{1}{c|}{62.8}         & 52.5         & 58.8         & 23.7         & \multicolumn{1}{c|}{45}           & 24.8         & 66.9         & 60.8         & \multicolumn{1}{c|}{50.9}         & 52.9                              \\
LLaVA-NeXT-Video~\cite{liu2024llavanext}                & \multicolumn{1}{c|}{7B}                               & 69.8         & 59.6         & 66.4         & 50.6         & 72.3         & 61.4         & \multicolumn{1}{c|}{63.3}         & 51.2         & 64.2         & 9.7          & \multicolumn{1}{c|}{41.7}         & 34.1         & 67.6         & 60.8         & \multicolumn{1}{c|}{54.2}         & 53.1                              \\ \hline
\multicolumn{18}{c}{\textbf{Open-Source   Streaming Video-LLMs}}                                                                                                                                                                                                                                                                                                                                                            \\ \hline
Flash-Vstream~\cite{zhang2025flash}                   & \multicolumn{1}{c|}{7B}                               & 25.5         & 32.1         & 29.3         & 33.7         & 29.7         & 28.8         & \multicolumn{1}{c|}{29.9}         & 36.4         & 33.8         & 5.9          & \multicolumn{1}{c|}{25.4}         & 5.4          & 67.3         & 60           & \multicolumn{1}{c|}{44.2}         & 33.2                              \\
VideoLLM-online~\cite{chen2024videollm}                 & \multicolumn{1}{c|}{8B}                               & 8.1          & 23.9         & 12.1         & 14           & 45.5         & 21.2         & \multicolumn{1}{c|}{20.8}         & 22.2         & 18.8         & 12.2         & \multicolumn{1}{c|}{17.7}         & -            & -            & -            & \multicolumn{1}{c|}{-}            & -                                 \\
Dispider~\cite{qian2025dispider}                        & \multicolumn{1}{c|}{7B}                               & 57.7         & 49.5         & 62.1         & 44.9         & 61.4         & 51.6         & \multicolumn{1}{c|}{54.5}         & 48.5         & 55.4         & 4.3          & \multicolumn{1}{c|}{36.1}         & 18           & 37.4         & 48.8         & \multicolumn{1}{c|}{34.7}         & 41.8                              \\
TimeChat-Online~\cite{yao2025timechat}                 & \multicolumn{1}{c|}{7B}                               & 69.8         & 48.6         & 64.7         & 44.9         & 68.3         & 55.4         & \multicolumn{1}{c|}{58.6}         & 53.9         & 62.8         & 9.1          & \multicolumn{1}{c|}{42}           & 32.5         & 36.5         & 40           & \multicolumn{1}{c|}{36.4}         & 45.6                              \\
StreamAgent~\cite{yang2025streamagent}                     & \multicolumn{1}{c|}{7B}                               & 71.2         & 53.2         & 63.6         & 53.9         & 67.3         & 58.7         & \multicolumn{1}{c|}{61.3}         & 54.8         & 58.1         & 25.8         & \multicolumn{1}{c|}{41.7}         & 35.9         & 48.4         & 52           & \multicolumn{1}{c|}{45.4}         & 49.4                              \\ \hline
Response-G1                     & \multicolumn{1}{c|}{8B}                               & 73.2         & 52.8         & 65.9         & 55.4         & 68.1         & 59.3         & \multicolumn{1}{c|}{62.5}         & 53.1         & 59.9         & 24.6         & \multicolumn{1}{c|}{45.9}         & 33.4         & 51.3         & 63.8         & \multicolumn{1}{c|}{49.5}         & 52.6                              \\ \hline
\end{tabular}
}
\caption{Performance comparison on OVO-Bench. Following the oofical benchmark settings, the Forward Active Responding subtask is implemented using \textit{proactive} iteraction mode, while all other subtasks follow the \textit{reactive} interaction mode.}
\label{table:ovobench}
\end{table*}







\begin{table}[t]
\centering
\Huge
\resizebox{1.0\linewidth}{!}{
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{ET-Bench}}                                                   \\ \cline{2-7} 
                                & \textbf{TVG\textsubscript{\textit{F1}}} & \textbf{TAL\textsubscript{\textit{Sim}}} & \textbf{DVC\textsubscript{\textit{F1}}} & \textbf{DVC\textsubscript{\textit{Sim}}} & \textbf{SLC\textsubscript{\textit{F1}}} & \textbf{SLC\textsubscript{\textit{Sim}}} \\ \hline
VideoLLM-online~\cite{chen2024videollm}                 & 13.2         & 9.1          & 24.0         & 13.4         & 9.9          & 10.1         \\
Dispider~\cite{qian2025dispider}                        & 36.1         & 27.3         & 33.8         & 18.9         & 18.8         & 12.4         \\
StreamBridge~\cite{wang2025streambridge}                    & 34.3         & 24.3         & 38.3         & 25.1         & 22.6         & 17.1         \\ \hline
\name                     & 33.8         & 28.1         & 32.5         & 24.9         & 24.2         & 18.8         \\ \hline
\end{tabular}
}
\caption{Performance comparison on ET-Bench.}
\label{table:etbench}
\end{table}
